The Differentiable Feasibility Pump

Although nearly 20 years have passed since its conception, the feasibility pump algorithm remains a widely used heuristic to find feasible primal solutions to mixed-integer linear problems. Many extensions of the initial algorithm have been proposed. Yet, its core algorithm remains centered around two key steps: solving the linear relaxation of the original problem to obtain a solution that respects the constraints, and rounding it to obtain an integer solution. This paper shows that the traditional feasibility pump and many of its follow-ups can be seen as gradient-descent algorithms with specific parameters. A central aspect of this reinterpretation is observing that the traditional algorithm differentiates the solution of the linear relaxation with respect to its cost. This reinterpretation opens many opportunities for improving the performance of the original algorithm. We study how to modify the gradient-update step as well as extending its loss function. We perform extensive experiments on MIPLIB instances and show that these modifications can substantially reduce the number of iterations needed to find a solution.

==> tables/ogvsp2.tex <==
\begin{table}[!ht]
	\centering
	\caption{\MC{need to format columns uniformly}}
	\label{tab:}
 \scalebox{0.7}{
	\begin{tabular}{cccc|ccc}
		\toprule
		INST & metric p2 & Feas p2 & Iters p2 & metric og & Feas og & Iters og\\ 
		\midrule
		academictimetablesmall & 0.5 & 0.00203 & 1000 & 0.5 & 0.00369 & 1000\\ 
		air05 & 0.0 & 0.0 & 4 & 4.44e-16 & 0.0 & 3\\ 
		app11 & 0.0611 & 1.34e-05 & 1000 & 0.0 & 0.0 & 137\\ 
		app12 & 6.76e-05 & 2.78e-09 & 18 & 6.76e-05 & 2.78e-09 & 18\\ 
		assign158 & 0.0 & 0.0 & 2 & 0.0 & 0.0 & 3\\ 
		b1c1s1 & 0.0 & 0.0 & 7 & 0.0 & 0.0 & 7\\ 
		beasleyC3 & 0.0 & 0.0 & 11 & 0.0 & 0.0 & 11\\ 
		binkar101 & 0.0 & 0.0 & 26 & 0.0 & 0.0 & 77\\ 
		blpar98 & 0.0 & 0.0 & 146 & 0.0 & 0.0 & 59\\ 
		blpic98 & 0.0 & 0.0 & 6 & 0.0 & 0.0 & 3\\ 
		bnatt400 & 0.497 & 0.00468 & 1000 & 0.475 & 0.00581 & 1000\\ 
		bppc408 & 0.0 & 0.0 & 3 & 0.0 & 0.0 & 2\\ 
		cbscta & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		chromaticindex10247 & 0.0 & 0.0 & 2 & 0.5 & 0.000629 & 1000\\ 
		chromaticindex5127 & 0.0 & 0.0 & 2 & 0.0 & 0.0 & 387\\ 
		cmflsp502488 & 0.427 & 0.000291 & 1000 & 0.0 & 0.0 & 16\\ 
		CMS7504 & 0.475 & 0.0 & 232 & 0.0 & 0.0 & 94\\ 
		cod105 & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		cost266UUE & 0.0 & 0.0 & 6 & 0.0 & 0.0 & 4\\ 
		csched007 & 0.0 & 0.0 & 683 & 0.333 & 0.00261 & 1000\\ 
		csched008 & 0.0 & 0.0 & 47 & 0.5 & 0.00609 & 1000\\ 
		cvs16r12889 & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		dano33 & 0.0 & 0.0 & 2 & 0.0 & 0.0 & 17\\ 
		dano35 & 0.0 & 0.0 & 4 & 0.0 & 0.0 & 7\\ 
		decomp2 & 0.5 & 0.00149 & 1000 & 0.5 & 0.00356 & 1000\\ 
		drayage10023 & 0.0 & 0.0 & 156 & 0.454 & 0.000357 & 1000\\ 
		drayage2523 & 0.0 & 0.0 & 292 & 0.475 & 0.000399 & 1000\\ 
		dws00801 & 0.38 & 0.000292 & 1000 & 0.166 & 0.000199 & 1000\\ 
		eil332 & 0.0 & 0.0 & 60 & 0.0 & 0.0 & 63\\ 
		eilA1012 & 0.0 & 0.0 & 356 & 0.422 & 0.00433 & 1000\\ 
		exp150055 & 0.0 & 0.0 & 2 & 0.0 & 0.0 & 3\\ 
		fast0507 & 0.0 & 0.0 & 5 & 0.0 & 0.0 & 5\\ 
		fastxgemmn2r6s0t2 & 0.0 & 0.0 & 38 & 0.0 & 0.0 & 35\\ 
		fhnwbinpack448 & 0.464 & 0.0253 & 1000 & 0.417 & 0.0252 & 1000\\ 
		glass4 & 0.0 & 0.0 & 15 & 0.0 & 0.0 & 50\\ 
		glasssc & 0.0 & 0.0 & 4 & 0.0 & 0.0 & 4\\ 
		gmu3540 & 0.0 & 0.0 & 26 & 0.0 & 0.0 & 8\\ 
		gmu3550 & 0.0 & 0.0 & 9 & 0.0 & 0.0 & 130\\ 
		graph20201rand & 0.0 & 0.0 & 31 & 0.0 & 0.0 & 16\\ 
		h80x6320d & 0.0 & 0.0 & 6 & 0.0 & 0.0 & 9\\ 
		irp & 0.0 & 0.0 & 23 & 0.0 & 0.0 & 42\\ 
		istanbulnocutoff & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		leo1 & 0.0 & 0.0 & 4 & 0.0 & 0.0 & 5\\ 
		leo2 & 0.0 & 0.0 & 3 & 0.0 & 0.0 & 4\\ 
		lotsize & 0.0 & 0.0 & 24 & 0.0 & 0.0 & 19\\ 
		mad & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		markshare2 & 0.0 & 0.0 & 6 & 0.0 & 0.0 & 6\\ 
		markshare40 & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		mas74 & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		mas76 & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		mc11 & 0.0 & 0.0 & 20 & 0.0 & 0.0 & 18\\ 
		mcsched & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		milov126r2401 & 1.11e-16 & 0.0 & 91 & 0.0 & 0.0 & 39\\ 
		momentum1 & 0.00014 & 5.55e-09 & 64 & 0.0021 & 3.77e-08 & 1000\\ 
		n2seq36q & 0.4 & 0.0 & 4 & 0.0 & 0.0 & 37\\ 
		n3div36 & 0.0 & 0.0 & 2 & 0.0 & 0.0 & 2\\ 
		neos1122047 & 0.111 & 0.0 & 7 & 0.3 & 0.0 & 25\\ 
		neos1171448 & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		neos1171737 & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		neos1445765 & 0.154 & 0.000287 & 1000 & 0.471 & 0.00352 & 1000\\ 
  		\bottomrule
	\end{tabular}
 }
\end{table}

 \begin{table}[!ht]
	\centering
	\caption{}
	\label{tab:22}
 \scalebox{0.7}{
  	\begin{tabular}{cccc|ccc}
		\toprule
		INST & metric p2 & Feas p2 & Iter p2 & metric og & Feas og & Iter og\\ 
		\midrule
		neos17 & 0.0 & 0.0 & 2 & 0.0 & 0.0 & 2\\ 
		neos2978193inde & 0.0 & 0.0 & 2 & 0.0 & 0.0 & 5\\ 
		neos2987310joes & 0.0 & 0.0 & 72 & 0.0 & 0.0 & 7\\ 
		neos3216931puriri & 0.479 & 0.00231 & 1000 & 0.5 & 0.00167 & 1000\\ 
		neos3627168kasai & 0.0 & 0.0 & 11 & 0.0 & 0.0 & 5\\ 
		neos3754480nidda & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		neos4300652rahue & 0.0 & 0.0 & 381 & 0.5 & 0.00314 & 1000\\ 
		neos4387871tavua & 0.375 & 0.0061 & 1000 & 0.5 & 0.0112 & 1000\\ 
		neos4763324toguru & 0.0 & 0.0 & 3 & 0.0 & 0.0 & 3\\ 
		neos4954672berkel & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		neos5093327huahum & 0.0 & 0.0 & 584 & 0.0 & 0.0 & 214\\ 
		neos5107597kakapo & 0.0 & 0.0 & 142 & 0.0184 & 3e-05 & 1000\\ 
		neos5188808nattai & 0.0 & 0.0 & 2 & 0.0 & 0.0 & 2\\ 
		neos5195221niemur & 0.5 & 0.000753 & 1000 & 0.5 & 0.0 & 89\\ 
		neos5 & 0.5 & 0.0 & 3 & 0.0 & 0.0 & 3\\ 
		neos827175 & 0.0 & 0.0 & 27 & 0.0 & 0.0 & 5\\ 
		neos860300 & 0.0 & 0.0 & 9 & 0.0 & 0.0 & 4\\ 
		neos911970 & 0.0 & 0.0 & 2 & 0.0 & 0.0 & 2\\ 
		neos933966 & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		neos957323 & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		neos960392 & 0.404 & 0.0 & 83 & 0.4 & 0.0 & 214\\ 
		net12 & 0.0833 & 0.0 & 12 & 0.5 & 0.0 & 10\\ 
		nexp1502085 & 0.0 & 0.0 & 6 & 0.0 & 0.0 & 6\\ 
		ns1116954 & 0.5 & 4.39e-05 & 1000 & 0.5 & 3.26e-05 & 1000\\ 
		ns1208400 & 0.5 & 0.00105 & 1000 & 0.491 & 0.000929 & 1000\\ 
		ns1830653 & 0.476 & 0.00105 & 1000 & 0.491 & 0.00185 & 1000\\ 
		opm2z10s4 & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		p200x1188c & 0.0 & 0.0 & 2 & 0.0 & 0.0 & 2\\ 
		pegsolitairea3 & 0.5 & 0.00115 & 1000 & 0.5 & 0.00106 & 1000\\ 
		pg534 & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		pg & 0.0 & 0.0 & 4 & 0.0 & 0.0 & 3\\ 
		pk1 & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		qap10 & 5.89e-13 & 0.0 & 2 & 1.67e-15 & 0.0 & 2\\ 
		rail507 & 0.0 & 0.0 & 5 & 0.0 & 0.0 & 4\\ 
		ran14x18disj8 & 0.0 & 0.0 & 8 & 0.0 & 0.0 & 5\\ 
		rdrplusc21 & 0.5 & 1.01e-05 & 1000 & 0.306 & 1.98e-05 & 1000\\ 
		reblock115 & 0.0918 & 0.0 & 50 & 0.229 & 0.0 & 29\\ 
		rmatr100p10 & 0.0 & 0.0 & 2 & 0.0 & 0.0 & 2\\ 
		rmatr200p5 & 0.0 & 0.0 & 2 & 0.0 & 0.0 & 9\\ 
		rocII511 & 0.268 & 4.4e-05 & 1000 & 0.139 & 1.5e-05 & 1000\\ 
		roi2alpha3n4 & 0.0 & 0.0 & 49 & 0.5 & 0.0022 & 1000\\ 
		satellites240 & 0.000401 & 7.07e-08 & 1000 & 0.5 & 2.98e-05 & 1000\\ 
		satellites260fs & 0.000326 & 5.15e-08 & 1000 & 0.5 & 0.000117 & 1000\\ 
		sct2 & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		seymour1 & 0.0 & 0.0 & 11 & 0.0 & 0.0 & 4\\ 
		seymour & 0.0 & 0.0 & 19 & 0.0 & 0.0 & 5\\ 
		sing326 & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		sing44 & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		sorrell3 & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		sp150x300d & 0.0 & 0.0 & 5 & 0.0 & 0.0 & 5\\ 
		sp97ar & 0.0 & 0.0 & 6 & 0.0 & 0.0 & 4\\ 
		sp98ar & 0.25 & 0.0 & 4 & 0.0 & 0.0 & 4\\ 
		supportcase18 & 0.0 & 0.0 & 98 & 0.473 & 0.00142 & 1000\\ 
		supportcase26 & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		supportcase40 & 0.0 & 0.0 & 2 & 0.0 & 0.0 & 2\\ 
		swath1 & 0.0 & 0.0 & 2 & 0.0 & 0.0 & 2\\ 
		swath3 & 0.0 & 0.0 & 4 & 0.0 & 0.0 & 3\\ 
		tbfpnetwork & 0.0 & 0.0 & 3 & 0.0 & 0.0 & 3\\ 
		thor50dday & 0.0 & 0.0 & 4 & 0.0 & 0.0 & 4\\ 
		tr1230 & 0.0 & 0.0 & 12 & 0.0 & 0.0 & 9\\ 
		trento1 & 0.0 & 0.0 & 3 & 0.0 & 0.0 & 3\\ 
		uccase12 & 0.0 & 0.0 & 3 & 0.0 & 0.0 & 3\\ 
		uccase9 & 0.5 & 0.000898 & 1000 & 0.0 & 0.0 & 4\\ 
		uctsubprob & 0.0 & 0.0 & 1 & 0.0 & 0.0 & 1\\ 
		unitcal7 & 0.475 & 0.000927 & 1000 & 0.457 & 0.000309 & 1000\\ 
		\bottomrule
	\end{tabular}
 }
\end{table}


==> tables/p2best.tex <==
\begin{table}[!ht]
	\centering
	\caption{}
	\label{tab:}
 \scalebox{0.7}{
	\begin{tabular}{cccccc}
		\toprule
		INST & $\eta$ & $\gamma$ & metric & Feas & Iters\\ 
		\midrule
		academictimetablesmall & 0.6 & 0.1 & 5.00e-01 & 2.03e-03 & 1000\\ 
		air05 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 4\\ 
		app11 & 0.6 & 0.1 & 6.11e-02 & 1.34e-05 & 1000\\ 
		app12 & 0.6 & 0.1 & 6.76e-05 & 2.78e-09 & 18\\ 
		assign158 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 2\\ 
		b1c1s1 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 7\\ 
		beasleyC3 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 11\\ 
		binkar101 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 26\\ 
		blpar98 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 146\\ 
		blpic98 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 6\\ 
		bnatt400 & 0.6 & 0.1 & 4.97e-01 & 4.68e-03 & 1000\\ 
		bppc408 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 3\\ 
		cbscta & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		chromaticindex10247 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 2\\ 
		chromaticindex5127 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 2\\ 
		cmflsp502488 & 0.6 & 0.1 & 4.27e-01 & 2.91e-04 & 1000\\ 
		CMS7504 & 0.6 & 0.1 & 4.75e-01 & 0.00e+00 & 232\\ 
		cod105 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		cost266UUE & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 6\\ 
		csched007 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 683\\ 
		csched008 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 47\\ 
		cvs16r12889 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		dano33 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 2\\ 
		dano35 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 4\\ 
		decomp2 & 0.6 & 0.1 & 5.00e-01 & 1.49e-03 & 1000\\ 
		drayage10023 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 156\\ 
		drayage2523 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 292\\ 
		dws00801 & 0.6 & 0.1 & 3.80e-01 & 2.92e-04 & 1000\\ 
		eil332 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 60\\ 
		eilA1012 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 356\\ 
		exp150055 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 2\\ 
		fast0507 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 5\\ 
		fastxgemmn2r6s0t2 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 38\\ 
		fhnwbinpack448 & 0.6 & 0.1 & 4.64e-01 & 2.53e-02 & 1000\\ 
		glass4 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 15\\ 
		glasssc & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 4\\ 
		gmu3540 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 26\\ 
		gmu3550 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 9\\ 
		graph20201rand & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 31\\ 
		h80x6320d & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 6\\ 
		irp & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 23\\ 
		istanbulnocutoff & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		leo1 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 4\\ 
		leo2 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 3\\ 
		lotsize & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 24\\ 
		mad & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		markshare2 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 6\\ 
		markshare40 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		mas74 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		mas76 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		mc11 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 20\\ 
		mcsched & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		milov126r2401 & 0.6 & 0.1 & 1.11e-16 & 0.00e+00 & 91\\ 
		momentum1 & 0.6 & 0.1 & 1.40e-04 & 5.55e-09 & 64\\ 
		n2seq36q & 0.6 & 0.1 & 4.00e-01 & 0.00e+00 & 4\\ 
		n3div36 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 2\\ 
		neos1122047 & 0.6 & 0.1 & 1.11e-01 & 0.00e+00 & 7\\ 
		neos1171448 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		neos1171737 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		neos1445765 & 0.6 & 0.1 & 1.54e-01 & 2.87e-04 & 1000\\ 
		neos17 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 2\\ 
  		\bottomrule
	\end{tabular}
  	\begin{tabular}{cccccc}
		\toprule
		INST & LR & LOSSREG & metric & Feas & Iter\\ 
		\midrule
		neos2978193inde & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 2\\ 
		neos2987310joes & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 72\\ 
		neos3216931puriri & 0.6 & 0.1 & 4.79e-01 & 2.31e-03 & 1000\\ 
		neos3627168kasai & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 11\\ 
		neos3754480nidda & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		neos4300652rahue & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 381\\ 
		neos4387871tavua & 0.6 & 0.1 & 3.75e-01 & 6.10e-03 & 1000\\ 
		neos4763324toguru & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 3\\ 
		neos4954672berkel & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		neos5093327huahum & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 584\\ 
		neos5107597kakapo & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 142\\ 
		neos5188808nattai & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 2\\ 
		neos5195221niemur & 0.6 & 0.1 & 5.00e-01 & 7.53e-04 & 1000\\ 
		neos5 & 0.6 & 0.1 & 5.00e-01 & 0.00e+00 & 3\\ 
		neos827175 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 27\\ 
		neos860300 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 9\\ 
		neos911970 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 2\\ 
		neos933966 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		neos957323 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		neos960392 & 0.6 & 0.1 & 4.04e-01 & 0.00e+00 & 83\\ 
		net12 & 0.6 & 0.1 & 8.33e-02 & 0.00e+00 & 12\\ 
		nexp1502085 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 6\\ 
		ns1116954 & 0.6 & 0.1 & 5.00e-01 & 4.39e-05 & 1000\\ 
		ns1208400 & 0.6 & 0.1 & 5.00e-01 & 1.05e-03 & 1000\\ 
		ns1830653 & 0.6 & 0.1 & 4.76e-01 & 1.05e-03 & 1000\\ 
		opm2z10s4 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		p200x1188c & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 2\\ 
		pegsolitairea3 & 0.6 & 0.1 & 5.00e-01 & 1.15e-03 & 1000\\ 
		pg534 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		pg & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 4\\ 
		pk1 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		qap10 & 0.6 & 0.1 & 5.89e-13 & 0.00e+00 & 2\\ 
		rail507 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 5\\ 
		ran14x18disj8 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 8\\ 
		rdrplusc21 & 0.6 & 0.1 & 5.00e-01 & 1.01e-05 & 1000\\ 
		reblock115 & 0.6 & 0.1 & 9.18e-02 & 0.00e+00 & 50\\ 
		rmatr100p10 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 2\\ 
		rmatr200p5 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 2\\ 
		rocII511 & 0.6 & 0.1 & 2.68e-01 & 4.40e-05 & 1000\\ 
		roi2alpha3n4 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 49\\ 
		satellites240 & 0.6 & 0.1 & 4.01e-04 & 7.07e-08 & 1000\\ 
		satellites260fs & 0.6 & 0.1 & 3.26e-04 & 5.15e-08 & 1000\\ 
		sct2 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		seymour1 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 11\\ 
		seymour & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 19\\ 
		sing326 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		sing44 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		sorrell3 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		sp150x300d & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 5\\ 
		sp97ar & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 6\\ 
		sp98ar & 0.6 & 0.1 & 2.50e-01 & 0.00e+00 & 4\\ 
		supportcase18 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 98\\ 
		supportcase26 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		supportcase40 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 2\\ 
		swath1 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 2\\ 
		swath3 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 4\\ 
		tbfpnetwork & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 3\\ 
		thor50dday & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 4\\ 
		tr1230 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 12\\ 
		trento1 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 3\\ 
		uccase12 & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 3\\ 
		uccase9 & 0.6 & 0.1 & 5.00e-01 & 8.98e-04 & 1000\\ 
		uctsubprob & 0.6 & 0.1 & 0.00e+00 & 0.00e+00 & 1\\ 
		unitcal7 & 0.6 & 0.1 & 4.75e-01 & 9.27e-04 & 1000\\ 
		\bottomrule
	\end{tabular}
 }
\end{table}

